Reference-Free Isotropic 3D EM Reconstruction using Diffusion Models

Electron microscopy (EM) images exhibit anisotropic axial resolution due to the characteristics inherent to the imaging modality, presenting challenges in analysis and downstream tasks.In this paper, we propose a diffusion-model-based framework that overcomes the limitations of requiring reference data or prior knowledge about the degradation process. Our approach utilizes 2D diffusion models to consistently reconstruct 3D volumes and is well-suited for highly downsampled data. Extensive experiments conducted on two public datasets demonstrate the robustness and superiority of leveraging the generative prior compared to supervised learning methods. Additionally, we demonstrate our method's feasibility for self-supervised reconstruction, which can restore a single anisotropic volume without any training data.

==> ablation_A.tex <==
\begin{table}[htb!]
\caption{Abalation for assumption of the degradation. The highest scores are highlighted in \textbf{bold}.}
\centering
\label{table:ablation_A}
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{4.0pt}
\scriptsize{
\begin{tabular}{|c|ccc|}
\hline
\textbf{Method} & PSNR$\uparrow$ & MS-SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\hline
Imputation& 25.06 & 0.802 & 0.495\\
\cline{1-4}
Gaussian, $\sigma=2$& 26.82 & 0.873 & 0.418\\
\cline{1-4}
Average& 26.91 & 0.878 & 0.415\\
\cline{1-4}
Interpolation& \textbf{27.55}& \textbf{0.901} & \textbf{0.391}\\
\hline
\end{tabular}
}
\end{table}


%\scriptsize{
%\begin{tabular}{|c|ccc|}
%\hline
%\textbf{method} & PSNR & MS-SSIM  & LPIPS \\
%\hline
%inpaint& 25.06 & 0.802 & 0.495\\
%\cline{1-4}
%gau $\sigma=2$& 26.82 & 0.873 & 0.418\\
%\cline{1-4}
%average& 26.91 & 0.878 & 0.415\\
%\cline{1-4}
%Ours& 27.55& 0.901 & 0.391\\
%\hline
%\end{tabular}
%}

==> ablation_consistency.tex <==
%\begin{table}[htb!]
%\centering
%\caption{Quantitative results on simulated anisotropic FIB25 dataset}
%\renewcommand{\arraystretch}{1.0}
%\setlength{\tabcolsep}{2.0pt}
%\scriptsize{
%\begin{tabular}{|r|ccc|}
%\hline
%\textbf{method} & PSNR & MS-SSIM  & LPIPS \\
%\hline
%inpaint& & & \\
%\cline{2-4}
%gau $\sigma=2$& & & \\
%\cline{2-4}
%average& & & \\
%\cline{2-4}
%Ours& & & \\
%\hline
%\end{tabular}
%}
%\end{table}


\scriptsize{
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{|c|}{\textbf{ZY}}  &\multicolumn{3}{|c|}{\textbf{ZX}} & \multicolumn{3}{|c|}{\textbf{XY}} \\
&PSNR & MS-SSIM & LPIPS & PSNR & MS-SSIM & LPIPS & PSNR & MS-SSIM & LPIPS \\
\hline
None&&&&&&&&& \\
\hline
Noise &&&&&&&&& \\
\hline
Ours&&&&&&&&& \\
\hline
\end{tabular}
}

==> ablation_table_fig.tex <==
\begin{figure}[htb!] 
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \renewcommand{\arraystretch}{2.0}
    \setlength{\tabcolsep}{2.0pt}
    \centering
    \caption{Quantitative results for comparing different assumptions of the degradation}
    \begin{tabular}{|c|ccc|}
    \hline
    \textbf{Method} & PSNR$\uparrow$ & MS-SSIM$\uparrow$  & LPIPS$\downarrow$ \\
    \hline
    Imputation& 25.06 & 0.802 & 0.495\\
    \cline{1-4}
    Gau $\sigma=2$& 26.82 & 0.873 & 0.418\\
    \cline{1-4}
    Average& 26.91 & 0.878 & 0.415\\
    \cline{1-4}
    Ours& 27.55& 0.901 & 0.391\\
    \hline
    \end{tabular}
    \label{fig:table}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{0.3\textwidth}
    \centering
    \caption{Visual compairsion of with/without considering consistency}    
    \includegraphics[width=\textwidth]{sample_img.png}
    \label{fig:image}
  \end{minipage}
\end{figure}

==> ablations_sum.tex <==
\begin{table}[htbp]
\caption{Ablation studies performed with simulated FIB-25 dataset. 
(Left): blind-PSF assumptions
(Right): with/without consistency sampling}
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{0.5pt}
\centering
\begin{tabular}{cc}
    \input{ablation_A.tex} & \input{ablation_consistency.tex}
\end{tabular}
\end{table}

==> fib25_factor4_table.tex <==

\begin{table}[tb]%[htb!]
\centering
\caption{Quantitative Comparison with other methods. Isotropic FIB25 volume is simulated to an anisotropic resolution of $64\times512\times512$. The baseline is linear interpolation. $\perp$ and $+$ indicate that the reconstruction was done on ZX slices or is ensembled, respectively.}
\label{table:comp}
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{0.3pt}
\scriptsize{
\begin{tabular}{|c|c|ccc|ccc|ccc|}
\hline
\multirow{3}{*}{\textbf{PSF}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{|c|}{\textbf{ZY}}  &\multicolumn{3}{|c|}{\textbf{ZX}} & \multicolumn{3}{|c|}{\textbf{XY}} \\
& & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\cline{2-11}
& Baseline & 26.12 & 0.842 & 0.567 & 26.11 & 0.840 & 0.555 & 26.18 & 0.848 & 0.379 \\
\cline{1-11}

\multirow{4}{*}{Exact} & 3D-SR-UNet\cite{3d_em} & \textbf{28.96} & \textbf{0.934} & 0.486 & \textbf{28.97} & \textbf{0.931} & 0.479 & \textbf{29.04} & \textbf{0.931} & 0.412\\
\cline{2-11}
& IsoNet\cite{fluroscence} & 28.62 & 0.928 & 0.490 & 28.56 & 0.924 & 0.495 & 28.67 & 0.922 & 0.328 \\
\cline{2-11}
& Ours & 27.92 & 0.914 & \textbf{0.375} & 27.93 & 0.916 & 0.434 & 28.03 & 0.913 & 0.296 \\
\cline{2-11}
& Ours\textsuperscript{$+$} & 28.39 & 0.924 & 0.426 & 28.39 & 0.922 & \textbf{0.425} & 28.49 & 0.920 & \textbf{0.264} \\
\hline



\multirow{6}{*}{Blind} & 3D-SR-UNet & 27.52 & 0.894 & 0.512 & 27.52 & 0.891 & 0.503 & 27.57 & 0.895 & 0.426 \\
\cline{2-11}
& IsoNet & 27.60 & 0.897 & 0.503 & 27.29 & 0.888 & 0.515 & 27.35 & 0.889 & 0.363 \\
\cline{2-11}
& Deng \textit{et al.}\cite{degradation_learning} & 27.65 & 0.901 & 0.496 & 27.65 & 0.901 & 0.504 & 27.75 & 0.900 & 0.408 \\
\cline{2-11}
& Ours & 27.55 & 0.901 & \textbf{0.391} & 27.55 & 0.903 & 0.448 & 27.64 & 0.901 & 0.325 \\
\cline{2-11}
& Ours\textsuperscript{$\perp$} & 27.57 & 0.905 & 0.453 & 27.57 & 0.900 & \textbf{0.393} & 27.66 & 0.901 & \textbf{0.280} \\
\cline{2-11}
& Ours\textsuperscript{$+$} & \textbf{27.95} & \textbf{0.911} & 0.431 & \textbf{27.95} & \textbf{0.909} & 0.433 & \textbf{28.04} & \textbf{0.908} & 0.284 \\
\hline
\end{tabular}
}
\end{table}

